Interaction of surface acoustic waves and magnetic thin films

Surface acoustic waves (SAWs) have emerged as innovative and energy-efficient means to manipulate domain walls (DWs) and skyrmions in thin films with perpendicular magnetic anisotropy (PMA) owing to the magnetoelastic coupling effect. This thesis focuses on the complex interplay between SAWs and magnetic thin films. The effects of the standing SAWs on the magnetisation dynamics in a Ta/Pt/Co/Ir/Ta thin film with PMA were first investigated. SAWs with frequency of 93.35 MHz significantly reduced the coercivity of the thin film by 21% and enhanced the magnetisation reversal speed by 11-fold. Standing SAWs introduce a dynamic energy landscape with a unique spatial distribution, forming striped domain patterns in the thin film. The use of rf signals for generating SAWs inevitably causes a heating effect in the device. This heating effect was examined in situ in a SAW device featuring a Ta/Pt/Co/Ta thin film with PMA using an on-chip platinum thermometer. The temperature increased by 10 K in the presence of SAWs at centre frequency of 48 MHz. The DW velocity was significantly enhanced in the presence of the standing SAWs by a factor of 4 compared to that with temperature change alone owing to the magnetoelastic coupling effect. To understand the SAW-enhanced DW motion, comprehensive micromagnetic simulations were performed on thin films in the presence of travelling SAWs. The findings highlighted that SAW-induced vertical Bloch lines within DWs can simultaneously boost DW depinning and dissipate energy at the DW via spin rotation. The SAW-induced strain gradient can be exploited to control skyrmion motion in a current-free manner. Micromagnetic simulations revealed that the use of orthogonal SAWs, combining horizontal travelling and vertical standing waves, offered a promising approach to direct skyrmion motion along desired trajectories, avoiding undesirable Hall-like motion.

==> Abbreviations/Abbreviations.tex <==
% Define your acronyms
\renewcommand*{\glstextformat}[1]{\textcolor{black}{#1}}

\newacronym[plural=Complementary metal-oxide-semiconductors, firstplural=complementary metal-oxide-semiconductors (CMOS)]{CMOS}{CMOS}{complementary metal-oxide-semiconductor}
\newacronym[plural=Co-planar waveguides, firstplural=co-planar waveguides (CPWs)]{CPW}{CPW}{co-planar waveguide}
\newacronym{dc}{dc}{direct current}
\newacronym{dcMS}{dcMS}{direct current magnetron sputtering}
\newacronym{DMD}{DMD}{digital micro-mirror device}
\newacronym{DMI}{DMI}{Dzyaloshinskii--Moriya interaction}
\newacronym[plural=Domain walls, firstplural=domain walls (DWs)]{DW}{DW}{domain wall}
\newacronym{FMR}{FMR}{ferromagnetic resonance}
\newacronym[plural=Interdigitated transducers, firstplural=interdigitated transducers (IDTs)]{IDT}{IDT}{interdigitated transducer}
\newacronym{LLG}{LLG}{Landau--Lifshitz--Gilbert}
\newacronym{MLA}{MLA}{maskless aligner}
\newacronym{MOKE}{MOKE}{magneto-optic Kerr effect}
\newacronym[plural=Prototype circuit boards, firstplural=prototype circuit boards (PCBs)]{PCB}{PCB}{prototype circuit board}
\newacronym[plural=Perpendicular magnetic anisotropies, firstplural=perpendicular magnetic anisotropies (PMAs)]{PMA}{PMA}{perpendicular magnetic anisotropy}
\newacronym{rf}{rf}{radio-frequency}
\newacronym[plural=Surface acoustic waves, firstplural=surface acoustic waves (SAWs)]{SAW}{SAW}{surface acoustic wave}
\newacronym[plural=Scattering parameters, firstplural=scattering parameters (S-parameters)]{S-parameter}{S-parameter}{scattering parameter}
\newacronym{SOC}{SOC}{spin--orbit coupling}
\newacronym{SOT}{SOT}{spin--orbit torque}
\newacronym{STT}{STT}{spin--transfer torque}
\newacronym[plural=Standing surface acoustic waves, firstplural=standing surface acoustic waves (SWs)]{SW}{SW}{standing surface acoustic waves}
\newacronym[plural=Travelling surface acoustic waves, firstplural=travelling surface acoustic waves (TWs)]{TW}{TW}{travelling surface acoustic waves}
\newacronym{UV}{UV}{ultraviolet}
\newacronym[plural=Vertical Bloch lines, firstplural=vertical Bloch lines (VBLs)]{VBL}{VBL}{vertical Bloch line}
\newacronym[plural=Vector network analysers, firstplural=vector network analysers (VNAs)]{VNA}{VNA}{vector network analyser}
\newacronym{XRR}{XRR}{X-ray reflectometry}
\newacronym{LED}{LED}{light-emitting diode}
\newacronym{SMA}{SMA}{SubMiniature version A}
